DeformerNet: A Deep Learning Approach to 3D Deformable Object Manipulation

In this paper, we propose a novel approach to 3D deformable object manipulation leveraging a deep neural network called DeformerNet. Controlling the shape of a 3D object requires an effective state representation that can capture the full 3D geometry of the object. Current methods work around this problem by defining a set of feature points on the object or only deforming the object in 2D image space, which does not truly address the 3D shape control problem. Instead, we explicitly use 3D point clouds as the state representation and apply Convolutional Neural Network on point clouds to learn the 3D features. These features are then mapped to the robot end-effector's position using a fully-connected neural network. Once trained in an end-to-end fashion, DeformerNet directly maps the current point cloud of a deformable object, as well as a target point cloud shape, to the desired displacement in robot gripper position. In addition, we investigate the problem of predicting the manipulation point location given the initial and goal shape of the object.

==> conclusion.tex <==
In this paper, we present a novel approach to controlling the shape of 3D deformable objects using a deep neural network (DNN) called DeformerNet. Our DeformerNet consists of two stages: the first stage utilizes CNN to map the point clouds to a compact 256-dimension feature vector, and the second employs a fully-connected neural network to map the feature vector to end-effector positions. In addition, we investigate the problem of detecting the manipulation point location.
